Shoulder of Dust Rings Formed by Planet-disk Interactions

Recent analyses of mm-wavelength protoplanetary disk observations have revealed several emission excesses on the previously identified dust rings, referred to as dust shoulders. The prevalence of dust shoulders suggests that they trace a common but unclear mechanism. In this work, we combine 3D, multifluid hydrodynamic simulations with radiative transfer calculations to explain the formation of dust shoulders. We find that the ring-shoulder pairs can result from the 3D planet-disk interactions with massive, gap-opening planets. The key driver is the dust filtration effect at the local pressure maximum due to planet-driven outward gas flows. Our work provides a possible explanation for the outer dust shoulders in recent super-resolution analyses of ALMA observations. It also provides insights into the formation of the inner dust shoulder in the PDS 70 disk and highlights the role of 3D effects in planet-disk interaction studies.

==> Table_2.tex <==
\begin{table}[t]
  \setlength\tabcolsep{0pt}
  \centering
  \caption{Parameter Space for RT Calculations}\label{tab:rt_param}\vspace{-8pt}
  \begin{tabular}{C{9}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}C{1}}
    \hline
    \multicolumn{1 }{C{9 }|}{\multirow{4}{*}{Star}}
  & \multicolumn{15}{C{15}|}{T Tauri (PDS 70)}
  & \multicolumn{15}{C{15} }{HAeBe (AB Aur)} \\
    \multicolumn{1 }{C{9 }|}{\hfill}
  & \multicolumn{15}{C{15}|}{$M_\star = 0.76 M_\odot$}
  & \multicolumn{15}{C{15} }{$M_\star = 2.36 M_\odot$} \\
    \multicolumn{1 }{C{9 }|}{\hfill}
  & \multicolumn{15}{C{15}|}{$D_\star = 1.26 D_\odot$}
  & \multicolumn{15}{C{15} }{$D_\star = 2.79 D_\odot$} \\
    \multicolumn{1 }{C{9 }|}{\hfill}
  & \multicolumn{15}{C{15}|}{$T_\star = 3972{\rm K}$}
  & \multicolumn{15}{C{15} }{$T_\star = 9770{\rm K}$} \\
    \hline
    \multicolumn{1}{C{9}|}{\multirow{2}{*}{Dust Mass}}
  & \multicolumn{6}{C{6}|}{\multirow{2}{*}{\textit{533}}}
  & \multicolumn{6}{C{6}|}{\multirow{2}{*}{\textit{543}}}
  & \multicolumn{6}{C{6}|}{\multirow{2}{*}{\textit{633}}}
  & \multicolumn{6}{C{6}|}{\multirow{2}{*}{\textit{643}}}
  & \multicolumn{6}{C{6} }{\multirow{2}{*}{\textit{654}}} \\
    \multicolumn{1}{C{9}|}{\hfill}
  & \multicolumn{6}{C{6}|}{\hfill} 
  & \multicolumn{6}{C{6}|}{\hfill}
  & \multicolumn{6}{C{6}|}{\hfill}
  & \multicolumn{6}{C{6}|}{\hfill}
  & \multicolumn{6}{C{6} }{\hfill} \\
    \hline
    \multicolumn{1 }{C{9 }|}{\multirow{2}{*}{Planet}}
  & \multicolumn{15}{C{15}|}{Saturn-like}
  & \multicolumn{15}{C{15} }{Jupiter-like} \\
    \multicolumn{1 }{C{9 }|}{\hfill}
  & \multicolumn{15}{C{15}|}{$3\times10^{-4}M_\star$}
  & \multicolumn{15}{C{15} }{$1\times10^{-3}M_\star$} \\
    \hline
    \multicolumn{1 }{C{9 }|}{\multirow{2}{*}{Beam Size}}
  & \multicolumn{10}{C{10}|}{25 mas}
  & \multicolumn{10}{C{10}|}{50 mas}
  & \multicolumn{10}{C{10} }{100 mas} \\
    \multicolumn{1 }{C{9 }|}{\hfill}
  & \multicolumn{10}{C{10}|}{(3.5 au)}
  & \multicolumn{10}{C{10}|}{(7 au)}
  & \multicolumn{10}{C{10} }{(14 au)} \\
    \hline
  \end{tabular}
  % \justify \vspace{-8pt}
  % \tablecomments{}
\end{table}
